On the Marginal Benefit of Active Learning: Does Self-Supervision Eat Its Cake?

Active learning is the set of techniques for intelligently labeling large unlabeled datasets to reduce the labeling effort. In parallel, recent developments in self-supervised and semi-supervised learning (S4L) provide powerful techniques, based on data-augmentation, contrastive learning, and self-training, that enable superior utilization of unlabeled data which led to a significant reduction in required labeling in the standard machine learning benchmarks. A natural question is whether these paradigms can be unified to obtain superior results. To this aim, this paper provides a novel algorithmic framework integrating self-supervised pretraining, active learning, and consistency-regularized self-training. We conduct extensive experiments with our framework on CIFAR10 and CIFAR100 datasets. These experiments enable us to isolate and assess the benefits of individual components which are evaluated using state-of-the-art methods (e.g.~Core-Set, VAAL, simCLR, FixMatch). Our experiments reveal two key insights: (i) Self-supervised pre-training significantly improves semi-supervised learning, especially in the few-label regime, (ii) The benefit of active learning is undermined and subsumed by S4L techniques. Specifically, we fail to observe any additional benefit of state-of-the-art active learning algorithms when combined with state-of-the-art S4L techniques.

==> algorithm.tex <==
	
%	\section{Algorithm}
	
%	\subsection{Active fixmatch with pretraining}
%	%\begin{figure}
%	%	\begin{tikzpicture}
%	%	\node at (0,0) {\includegraphics[scale=1]{figs/heatmap}};
%	%	\end{tikzpicture}
%	%\end{figure}
%	
%	\begin{algorithm}
%		\SetAlgoLined
%		%\SetKwRepeat{While}{While}{end}%
%		\textbf{Input}: DCL pre-train model $\bth_{0}$ and $\bth_{1}$, $f(\bth)$ is the feature representation, $p(\bth)$ is the prediction after softmax. Unlabeled training dataset $\UL$, number of classes $n$, $n$ labeled samples $(\X,\y)=\{(\x_{i},y_{i})\}_{i=1}^n$ where each class has 1 labeled sample. Active learning budget at each active learning epoch $b$, active learning interval $k$, maximum active learning samples $b_{max}$, an oracle $O$. Threshold $r$\;
%		\textbf{Initialization}: $e=1$\;
%		\While{$e<MaxEpoch$}{
%			$\bth_0$=Fixmatch($\X,\y,\textbf{U},\bth_0$)\;
%			$\bth_1$=Fixmatch($\X,\y,\textbf{U},\bth_1$)\;
%			
%			\If{e mod k=0 \textbf{and} $|X|<b_{max}$}{
%				$\F_0=f(\bth_1,\UL)$\;
%				$\F_1=f(\bth_2,\UL)$\;
%				\textbf{score}=$\textbf{0}_n$\;
%				$\X'=\phi$\;
%				\For{$m\gets0$ \KwTo $1$}{
%					$\textbf{Labels},\textbf{Centers}=$Same-size k-Means$(F_m,n)$\;
%					We can use fixmatch output rather than clustering \;
%					\For {$c\gets1$ \KwTo $n$}{
%						$\UL'=\UL[$argsort$($norm$(\F_{m}-\textbf{Centers}_c))[${\normalfont 0:r}$]]$\;
%						$\textbf{Centers}'_{c}=$mean$(f(\bth_{1-m},U'))$\;
%						$std_c'=$norm$($std$(f(\bth_{1-m},U_{Labels=c})))$\;
%						
%						\For {$i\gets1$ \KwTo $n$}{
%							$\textbf{score}_c+=$max($-\log($distance$(\textbf{Centers}'_{c}$,$\textbf{Centers}'_{i})/std_c')$,0) \quad $(c\neq j)$\;
%						}
%					}
%				}
%				\textbf{SampleNumber}=round$(b*\textbf{score})$\;
%				\For {$c\gets1$ \KwTo $n$}{
%					$\X'=\X'\cup$ core-set$(U_{Labels=c},SampleNumber_c,F_{1-m})$\;
%				}
%				$\y'=oracle(\X')$\;
%				$\UL=\UL-\X'$\;
%				$(\X,\y)=(\X,\y)\cup (\X',\y')$\;
%			}
%		}
%		\caption{Active Fixmatch on DCL pretrain AC3}
%
%	
%	
%	\begin{itemize}
%		\item On datasest $\{\x,y\}^{n}$, use DCL pre-trained model $\M_0$, $\M_1$ whose parameter can be vectorized as $\bth_0$ and $\bth_1$ to extract feature representation $f_0(\X)=\M_0(\X,\bth_0)$, $f_1(\X)=\M_1(\X,\bth_1)$
%		\item Cluster $f_0(\X)$ by k-means, let us denote the $k$ indices which nearest to each cluster center $i$ as $S_i\subset[n]$ and $|S|=k$
%		\item Compute centers of each cluster $S_i$ using features from $\M_1$, which is $c_i=\text{mean}(f_1(\X_{S_i}))$
%		\item Measure the divergence of each cluster under the new feature representation (e.g std, angle) and decide the number of samples for labeling.$sqrt(std_i*std_j) / dist_{i,j}$ 
%		
%		$(std_i+std_j) / dist_{i,j}$
%		\item $\sum_j^n{-log(distance_{i,j})}$
%	\end{itemize}
%	
%	
%	
%		\end{algorithm}
